PQCAD-DM: Progressive Quantization and Calibration-Assisted Distillation for Extremely Efficient Diffusion Model

Diffusion models excel in image generation but are computational and resource-intensive due to their reliance on iterative Markov chain processes, leading to error accumulation and limiting the effectiveness of naive compression techniques. In this paper, we propose PQCAD-DM, a novel hybrid compression framework combining Progressive Quantization (PQ) and Calibration-Assisted Distillation (CAD) to address these challenges. PQ employs a two-stage quantization with adaptive bit-width transitions guided by a momentum-based mechanism, reducing excessive weight perturbations in low-precision. CAD leverages full-precision calibration datasets during distillation, enabling the student to match full-precision performance even with a quantized teacher. As a result, PQCAD-DM achieves a balance between computational efficiency and generative quality, halving inference time while maintaining competitive performance. Extensive experiments validate PQCAD-DM's superior generative capabilities and efficiency across diverse datasets, outperforming fixed-bit quantization methods.

==> preliminaries/challenge.tex <==
\subsection{Challenge Analysis} 

We recognize two challenges that arise during compression due to iterative denoising processes in the Diffusion model: the fluctuating activation distribution as time steps, and the sampling inference errors that accumulate due to fusion compression.

\noindent \textbf{Variation of activation distribution}  
%considering that diffusion models use the same noise estimation network to process inputs at all time steps, the output distribution of the noise estimation network at each time step produces different activation distributions.
The output distribution of the noise estimation network at each time step is significantly different, resulting in a vibrating activation distribution. 
%그림에서 볼 수 있듯이 각 시간 단계에서 노이즈 추정 네트워크의 출력 분포는 크게 다르므로 진동하는 활성화 분포가 발생합니다.
At an arbitrary time step \( t \), the input to the diffusion model is derived from the output \( \bfx_{t+1} \) of the diffusion model at the previous time step \( t+1 \), operating iteratively across all time steps \( T \).
%임의의 시간 단계 t에서 노이즈 추정 모델의 입력은 이전 시간 단계 t+1에서 확산 모델의 출력인 xt+1에 의해 유도 되며 모든 시간 단계 T를 곱한 만큼 반복적인 과정 작동합니다. 
This results in the activation distribution of the same noise estimation model differing at each step due to varying inputs over time (as shown in Fig.~\ref{fig:challenge} (b)).
%이는 동일한 노이즈 추정 모델에 모든 시간 스텝에서 다른 입력으로 인한 활성화의 분포가 다름을 발생시킨다. 
In particular, activations in certain layers are distributed significantly differently depending on the time step during training.
%특히 특정 계층에서의 활성화는 훈련 중 시간 스텝에 따라 크게 다르게 분포한다. 
The characteristics of this distribution show that the quantization error between full-precision activations and activations quantized using the ANN quantization method accumulates over timesteps during the sampling process, making it challenging to generate high-performing DMs.
%이런 분포의 특성은 전체 정밀도 활성화와 정적으로 양자화된 활성화 사이의 오류가 샘플링 프로세스 동안 시간 단계에 걸쳐서 양자화 오류 누적되어 성능이 우수한 DMs을 생성하기 어려움을 관찰했습니다.

\noindent \textbf{Compression error accumulation} 
To expand the versatility of DMs, the fused compression approach that simply incorporates neural network quantization~\cite{ptq4dm,q-diff,tfmq} and distillation~\cite{progressivedistill,progressivedistill2} further accelerates error accumulation.
%DMs의 범용적 사용 가능성을 넓히고자 신경망 양자화와 신경망 증류를 단순히 추가한 복합적인 압축은 더욱 오류 누적이 가속화됩니다. 
%At an arbitrary time step \( t \), the input to the diffusion model is derived from the output \( \bfx_{t+1} \) of the diffusion model at the previous time step \( t+1 \), operating iteratively across all time steps \( T \).
%임의의 시간 단계 t에서 노이즈 추정 모델의 입력은 이전 시간 단계 t+1에서 확산 모델의 출력인 xt+1에 의해 유도 되며 모든 시간 단계 T를 곱한 만큼 반복적인 과정 작동합니다. 
%Neural network quantization introduces noise to activations and weights, leading to layer-wise errors that accumulate over the continuous time steps of diffusion models, resulting in amplified quantization errors in later stages.
Applying neural network quantization to a model causes noise to the activation and weight of the pre-trained model, resulting in quantization errors in the outputs of each layer.
Moreover, the continuous time steps of the diffusion model are another source of cumulative errors, where small errors in the earlier time steps accumulate into larger quantization errors in the later stages.
%더욱이, 확산 모델의 연속적인 시간 스텝은 또 다른 축의 오류 누적의 원인이며 전반 시간의 조금한 오류가 후반 시간 단계로 갈수록 큰 양자화 오류로 누적이 됩니다. 
On the other hand, the quality of the teacher model in the diffusion distillation process is a crucial factor in maintaining the performance of the student model. The diffusion distillation process relies on mapping the two-step denoised output of the teacher model to the one-step output of the student model, making the quality of the teacher model essential for preserving the student model's performance.
%반면, 확산 증류 과정의 교사 모델 품질은 학생 모델의 성능에 유지에 중요한 요소입니다. 확산 증류 과정은 오직 교사 모델의 2 step 디노이징한 출력과 학생 모델의 한 스텝 출력을 메핑하는 방법으로써 교사 모델의 품질은 학생 모델의 성능 유지를 위한 중요 요소입니다. 

However, simply applying the two compression methods sequentially fails to minimize the quantization error of the diffusion model, and distilling from a quantized teacher model with degraded quality further causes severe compression errors in the student model.
%하지만, 두 압축 방법을 단순히 연속적으로 적용하면 확산 모델의 양자화 오류를 최소화 못하고, 양자화되어 품질이 악화된 교사 모델을 증류를 함으로 학생 모델은 압축 오류가 심각하게 발생합니다.
As shown in Figure 3, the MSE distance measuring the compression error of the DM fused with both compression methods exhibits a noticeable increase with the reduction of sampling time steps, compared to the low-bit quantized DM. This indicates that the accumulation of quantization errors becomes more pronounced as the noise removal process progresses from early to later time steps, with significant errors compounding over time.
%그림 3에서 볼 수 있듯이, 저비트로 양자화된 DM의 압축 오류보다 두 압축 방법을 fusion시킨 DM의 압축 오류를 측정한 MSE 거리는 샘플링 시간 단계의 감소와 함께 눈에 띄는 증가를 보입니다. 이는 노이즈 제거 프로세스가 초기 시간부터 크게 누적되는 오류가 나중 시간 단계로 이동함에 따라 양자화 오류의 누적이 더욱 두드러진다는 것을 의미합니다.
%%뒤에 데이터 셋에서 시간 분포에서 활성화를 최대한 일치 시키기 위해서 시간단계로 양자화 했다!!!!!
%%%%%%%%%
%Diffusion model's noise estimation neural network quantization and neural network distillation perturb the weights and activations, causing errors in the output values of each layer.
%DMs의 잡음 추정 신경망 양자화와 신경망 증류는 가중치와 활성화에 교란을 일으켜 각 계층의 출력값에 오류를 발생시킵니다.
%Previous studies ~\cite{q-diff, tfmq} have found that error accumulation across multiple layers makes it difficult to maintain performance after quantization with low precision, and attempts to mitigate this by observing the dynamic nature of activation in diffusion models and sampling calibration datasets throughout the entire time step.
%이전 연구[q-diffusion]에서는 여러 계층 걸쳐 오류 누적되는 경향이 있어서 낮은 정밀로 양자화한 후 성능을 유지 하는 것은 어려움으로, 확산 모델에서 활성화의 동적 특성을 보고하고 전체 시간 프레임에 걸쳐 보정 데이터 세트를 샘플링하여 이를 해결하려고 시도했습니다.
%Another axis of study~\cite{progressivedistill} suggests that incremental distillation can significantly accelerate the inference speed of diffusion models by reducing the accumulation of radical knowledge gaps between the two models.
%또 다른 연구[00]에 따르면 점진적 증류는 정보 격차의 축적을 줄여 확산 모델의 추론 속도를 크게 가속화할 수 있습니다. 
%However, in order to broaden the general usability of diffusion models, we found that the fusion compression method, which simply adds neural network quantization and distillation for high compression, accelerates the accumulation of compression errors.
%하지만, 우리는 확산 모델의 범용적 사용 가능성을 넓히고자 Superior 압축을 위하여 신경망 양자화와 신경망 증류를 단순히 추가한 복합적인 압축은 더욱 오류 누적이 가속화됨을 발견했습니다.
%As shown in Fig.~\ref{fig:layer error}, the MSE distance measuring the compression error of low-bit quantized DM shows a significant increase with a decrease in the sampling time step. 
%Furthermore, the straightforward post neural-network distillation quantization process results in the accumulation of even larger compression errors. 
%This means that the accumulation of fusion compression errors becomes more pronounced as the denoising process largely accumulates from the initial time moves to the later time step.
%그림 2에서 볼 수 있듯이, 저비트로 양자화된 DM의 양자화 오류를 측정한 MSE 거리는 샘플링 시간 단계의 감소와 함께 눈에 띄는 증가를 보입니다. 이는 노이즈 제거 프로세스가 초기 시간부터 크게 누적되는 오류가 나중 시간 단계로 이동함에 따라 양자화 오류의 누적이 더욱 두드러진다는 것을 의미합니다. 

